An unbiased approach to compressed sensing

In compressed sensing a sparse vector is approximately retrieved from an under-determined equation system $Ax=b$. Exact retrieval would mean solving a large combinatorial problem which is well known to be NP-hard. For $b$ of the form $Ax_0+\epsilon$ where $x_0$ and $\epsilon$ is noise, the `oracle solution' is the one you get if you a priori know the support of $x_0$, and is the best solution one could hope for. We provide a non-convex functional whose global minimum is the oracle solution, with the property that any other local minimizer necessarily has high cardinality. We provide estimates of the type $\|\hat x-x_0\|_2\leq C\|\epsilon\|_2$ with constants $C$ that are significantly lower than for competing methods or theorems, and our theory relies on soft assumptions on the matrix $A$, in comparison with standard results in the field. The framework also allows to incorporate a priori information on the cardinality of the sought vector. In this case we show that despite being non-convex, our cost functional has no spurious local minima and the global minima is again the `oracle solution', thereby providing the first method which is guaranteed to find this point for reasonable levels of noise, without resorting to combinatorial methods.

==> suppl_mat_unbiased_nobeta.tex <==
\newpage


\begin{center}
{\Large \bf Proofs and further results\par}
\vspace*{24pt}
\end{center}
\iffalse
\section{Relaxation and the $\S_\gamma$-transform}\label{regS}
Let $f$ be any $[0,\infty]-$valued functional on $\R^n$, $\C^n$ or for that matter any separable Hilbert space $\H$. The $\S_{\gamma}$-transform, where $\gamma>0$ is a parameter, is designed such that $\S^2_{\gamma}(f)(x)+\frac{\gamma}{2}\|x\|_2^2$ is the l.s.c. convex envelope of $f(x)+\frac{\gamma}{2}\|x\|_2^2$. It can be shown that $\S^2_\gamma(f)$ is continuous wherever it is finite, and that $\gamma$ is the maximum negative curvature of $\S^2_\gamma(f)$. It also holds that $\S^2_\gamma(f)(x)$ increase with increasing $\gamma$, that $\lim_{\gamma\rightarrow\infty}\S^2_{\gamma}(f)=f$ and that $\lim_{\gamma\rightarrow 0^+}\S^2_{\gamma}(f)$ equals a convex minorant above the l.s.c. convex envelope of $f$, which in the cases considered here is identically 0.


Its potential use as a regularizer for problems of the form \eqref{genprob}, i.e. replacing $f(x)+\frac{1}{2}\|A x-b\|_2^2$ with
\begin{equation}
\S^2_\gamma(f)(x)+\frac{1}{2}\|A x-b\|_2^2,
\label{rep}
\end{equation}
was investigated in [...] After much discussion we decided to fix $\gamma=2$ and remove the traditional factor $\frac{1}{2}$ in this paper, since it substantially simplifies formulas. This is not a limitation since one can always obtain a such a problem by rescaling $f,~ A$ and $b$.
To see that this can be done, note that a simple computation shows $\S_\gamma^2(f)=\frac{\gamma}{2}\Q_2(\frac{2}{\gamma}f)$ (see [..]) so that \eqref{rep} is equivalent to $$\Q_2(\frac{2}{\gamma}f)(x)+\fro{\frac{A x}{\sqrt{\gamma}}-\frac{b}{\sqrt{\gamma}}}.$$

We henceforth assume that such a rescaling has been done so that we are interested in minimizing
\begin{equation}\label{relax}\K_{reg}(x)=\Q_2(f)(x)+\fro{{A x-b}}\end{equation} instead of $\K(x)=f(x)+\fro{A x-b}$.
%In this setting, the main result of [...] stipulates that, as long as $\|A\|<1$, the local minimizers of $\K_{reg}$ is a subset of those of $\K$, and most importantly that the global minimizers coincide. The restriction $\|A\|<1$ is too restrictive for the setting considered here, since we want $A$ to have normalized columns. Luckily, as we will show in Theorems \ref{celok5} and \ref{celok6}, the same conclusion holds under looser assumptions for the particular cases $f=\card$ and $f=\iota_{P_k}$.
\fi



\section{Uniqueness of minimizers and stationary points with the desired property}\label{sec:unique}
We now turn to the heart of the matter, namely uniqueness of sparse minimizers of $\K_{reg}$, more precisely minimizers in a given $k$-sparse set $P_k$.
As noted in the introduction, this is not possible without imposing additional conditions on $A$ as well as $b$. In this section we provide such a condition and in the coming ones we show what it entails in practice for the sparsity (and $k$-sparsity) problem.

We recall that the \emph{subdifferential} of a function \( g  \) is the set-valued operator \( \partial g \) defined by \[ \partial g (x) = \{ u \, : \, g(y) \ge g(x) + \langle u , y -x \rangle \ \forall \, y  \}. \] The elements of \( \partial g (x)  \) are the \emph{subgradients} of \(g\) at \( x\).

We say that a point $x$ is a stationary point of $g$ if $0\in \partial g(x)$. For the case when $g$ is a sum of a convex function $g_c$ and a differentiable function $g_d$, it is easy to see that $x$ is a stationary point if and only if $-\nabla g_d(x)\in \partial g_c(x)$ where $\partial g_c(x)$ denotes the usual subdifferential. Set \begin{equation}\label{gdef}\G(x)=\frac{1}{2}\Q_2(f)(x)+\frac{1}{2}\fro{x},\end{equation} i.e. $2\G$ the l.s.c. convex envelope of $f(x)+\fro{x}$.
We have
\begin{equation}\label{fr3}\K_{reg}(x)=2\G(x)-\fro{x}+\fro{Ax-b}\end{equation}
which upon differentiation yields that $x'$ is a stationary point of $\K_{reg}$ if and only if
\begin{equation}\label{sp}(I-A^* A)x' + A^* b\in\partial \G(x').\end{equation}
Given any $x$, we therefore associate with it a new point $z$ via
\begin{equation}\label{y}
z=(I-A^* A)x + A^* b.
\end{equation}
The importance of $z$ is due to the following simple observation.

\begin{proposition}\label{thm:statpoint}
Let $x'$ and $x''$ be distinct stationary points of $\K_{reg}$ such that $x''-x'\in P_k$. Then
\begin{equation}\label{ineq}\re\scal{z''-z',x''-x'}\leq \delta_k^-\fro{x''-x'}.\end{equation}
\end{proposition}

The above proposition will mainly be used backwards, i.e.~we will show that \eqref{ineq} does not hold and thereby conclude that $x''-x'\not\in P_k$.

\begin{proof}
We have $$z''-z'=( I-A^* A)x''+A^*b-( I-A^* A)x'-A^*b=(I-A^* A)(x''-x'),$$
so taking the scalar product with $x''-x'$ gives $$\re\scal{z''-z',x''-x'}=\fro{x''-x'}-\fro{A(x''-x')}\leq \delta_k^-\fro{x''-x'},$$ as desired. Note that it is not necessary to take the real part, but we leave it since scalar products in general can be complex numbers.
\end{proof}

As we shall see, the point $z'$ has a decisive influence on the coming sections. To begin with, it has the following interesting property.

\begin{proposition}
A point $x'$ is a stationary point of $\K_{reg}$ if and only if it solves the convex problem $$x'\in\argmin_x \Q_2(f)(x)+\fro{x-z'}.$$
\end{proposition}
Note the absence of $A$ in the above formula, which in particular implies that $\Q_2(f)(x)+\fro{x-z'}$ is the convex envelope of $f(x)+\fro{x-z'}$.
\begin{proof}
As noted in \eqref{sp}, $x'$ is a stationary point of $\K_{reg}$ if and only if $z'\in\partial\G(x')$. By the same token, $x'$ is a stationary point of $$\Q_2(f)(x)+\fro{x-z'}=2\G(x)-2\scal{x,z'}+\fro{z'}$$ if and only if $z'\in\partial\G(x')$, and since the functional is convex (and clearly has a well defined minimum) the stationary points coincide with the set of minimizers.
\end{proof}


\section{The sparsity problem}\label{seccard}

We return to the sparsity problem, and consider $f(x)=\mu\card(x)$ where $\mu$ is a parameter and $\card (x)$ is the number of non-zero entries in the vector $x$. In this case we have,
\begin{equation}\label{l0000}\Q_2(\mu\card)(x)=\sum_{j=1}^n \mu-\para{\max\{\sqrt{\mu}-{ |x_j|},0\}}^2, \quad x\in\R^n.\end{equation}
To recapitulate, we want to minimize \eqref{q1}, i.e.~\begin{equation}\label{t57}\kfi(x)=\mu\card(x)+\fro{Ax-b}\end{equation} which we replace by \eqref{q1reg}, i.e. \begin{equation}\label{fr2}\kfir(x)=\Q_2(\mu\card)(x)+\fro{Ax-b}.\end{equation}

\subsection{Equality of minimizers for $\kfi$ and $\kfir$}

As noted by Aubert, Blanc-Feraud and Soubies (see Theorems 4.5 and 4.8 in \cite{soubies-etal-siims-2015}),
$\kfir$ has the same global minima and potentially fewer local minima than $\kfi$ if \begin{equation}\label{alpha}\|A\|_{\infty,col}=\sup_i \|a_i\|_2\leq 1,\end{equation} where $a_i$ denotes the columns of $A$. Below we (essentially) reproduce their statement in the terminology of this paper, and also include a proof for completeness.

\begin{theorem}\label{celok5}
If $\|A\|_{\infty,col}<1$, then any local minimizer of $\kfir$ is a local minimizer of $\kfi,$ and the (nonempty) set of global minimizers coincide. If merely $\|A\|_{\infty,col}=1$, then any connected component of global minima of $\kfir$ includes at least two global minima of $\kfi$.
\end{theorem}

\begin{proof}
We first establish that $\inf \kfi=\inf \kfir$. Since $\kfi\geq \kfir$ it suffices to show that $\inf \kfi\leq \inf \kfir$. Suppose not and let $x_0$ be a point such that $\kfir(x_0)<\inf \kfi$. Then there must be some index $j$ such that the corresponding value in $\Q_2(\mu\card)(x_0)$ is different from $\mu\card (x_{0,j})$, which (see \eqref{l0000}) implies that \begin{equation}\label{py1}0<|x_{0,j}|<\sqrt\mu.\end{equation} But then \begin{equation}\label{py}\partial_{x_{0,j}}^2\kfir(x_0)=-2+2\|a_j\|_2^2\leq 0.\end{equation} It follows that we can redefine $x_{0,j}$ to equal either $0$ or $\sqrt{\mu}$, so that the resulting point $x_1$ satisfies $\kfir(x_1)\leq \kfi(x_0)$. We can now continue like this for another index $j$ such that \eqref{py1} holds (if it exists), and this process must terminate after finitely many steps $N$. Denoting the resulting point by $x_N$, we see that it satisfies $\kfi(x_N)=\kfir(x_N)<\inf \kfi$, a contradiction.

It is easy to see that $\kfi$ has global minimizers, and by the above argument these are also global minimizers for $\kfir$. Now let $x_0$ be a global minimizer of $\kfir$ but not for $\kfi$. As before we have that \eqref{py1} and \eqref{py} holds for some index $j$, and we clearly must have equality in the latter. If $\|A\|_{\infty,col}<1$ this is a contradiction, and hance we see that the global minimizers of $\kfi$ and $\kfir$ coincides. If merely $\|A\|_{\infty,col}=1$, then we can redefine $x_{0,j}$ to equal either $0$ or $\sqrt{\mu}$ without changing the value of $\kfir$, and as before this process eventually leads to a point $x_N$ which is also a global minimizer for $\kfi.$ By the construction, there are at least two such points.

It remains to prove the statement about local minimizers. If $x_0$ is a local minimizer of $\kfir$ and $\|A\|_{\infty,col}<1$, we immediately get a contradiction from \eqref{py} unless $\kfi(x_0)=\kfir(x_0)$. In view of $\kfi\geq \kfir$, this establishes the claim.
\end{proof}






%Although many of the results below can be extended to situations where this constraint does not hold, we will for the remainder assume this, since the text becomes much easier to read.

%In fact, this estimate can be improved slightly by replacing $\|A\|$ by the smaller number $\beta_1$. We collect this and a few other observations in the coming subsection.
%
%\subsection{Original vs. relaxed functional}
%The following theorem is taken from \cite{}.
%\begin{theorem}\label{celo12}
%Let $2>(\beta_1)^2$. If $x_l$ is a local minimizer (resp. strict local minimizer) of $\kfir$, then it is also a local minimizer (resp. strict local minimizer) of $\kfi$, and $\kfi(x_l)=\kfir(x_l)$. Moreover \begin{equation}\label{1}x_{l,j}\not \in \Big(0,\sqrt{\mu}\Big).\end{equation} Finally, the sets of global minimizers of $\kfi$ and $\kfir$ are nonempty and coincide.
%\end{theorem}
%
%If the condition $2> (\beta_1)^2$ fails, we may still have a $p\geq 1$ such that $\gamma>(\beta_{p+1})^2$. In this situation, we have the following weaker version of Theorem \ref{celo1}.
%
%\begin{theorem}\label{celo2}
%Let $2>(\beta_{p+1})^2$. If $x_l$ is a local minimizer of $\kfir$, then \eqref{1} can fail for at most $p$ values $x_{l,j}$ of $x_l$. If \eqref{1} holds for all $x_{l,j}$, equivalently if $\kfir(x_l)=\kfi(x_l)$, then $x_l$ is also a local minimizer of $\kfi$. In particular, if $x_l$ is a global minimizer of $\kfir$, then it is a global minimizer of $\kfi$.
%\end{theorem}
%\begin{proof}
%Suppose that \eqref{1} fails for $p+1$ indices, and let $\v$ be a vector that is nonzero at those indices and moreover such that $\|A\v\|^2<\gamma\|\v\|^2,$ which exists by the definition of $\beta_{p+1}$ and the assumption $\gamma>\beta_{p+1}^2$. Then the function $t\mapsto \kfir(x_l+t\v)$ is easily seen to have second derivative at $t=0$ equal to $-\gamma\|\v\|^2+\|A\v\|^2,$ which is negative. This contradicts that $x_l$ is a local minimizer and hence proves that \eqref{1} indeed must hold. The final statements are immediate by the inequality $\kfir\leq \kfi$.
%\end{proof}
%


\subsection{On the uniqueness of sparse stationary points}\label{erai}
%Given subset $S\subset\{1,\ldots,n\}$ we define $A_S$ to be the matrix whose columns are $a_j$ for $j\in S$ and $0$ else.
Next we take a closer look at the structure of the stationary points. Given $N$ such that $\delta_{N}^-<1$, we will show that under certain assumptions the difference between two stationary points always has at least $N$ elements.
Hence if we find a stationary point with less than $N/2$ elements then we can be sure that this is the sparsest one. The main theorem reads as follows:


\begin{theorem}\label{thm:statpoint:vec}
Let $x'$ be a stationary point of $\kfir$, let $z'$ be given by \eqref{y}, and assume that
\begin{equation}\label{e4}|z_i'|\not\in\left[{(1-\delta_N^-)}{\sqrt{\mu}},\frac{{\sqrt{\mu}}}{1-\delta_N^-}\right]\end{equation} for all $i\in\{1,\ldots,n\}$.
If $x''$ is another stationary point of $\kfir$ then $\card(x''-x') > N$.
\end{theorem}

%With $N=2k$ we get the following corollary.

%\begin{corollary}\label{cor:statpoint:vec}
%Let $x'$ be a stationary point of $\kfir$, let $z'$ be given by \eqref{y}, and assume that
%\begin{equation}\label{e4c}|z_i'|\not\in\left[{\beta_{2k}^2}{\sqrt{\mu}},\frac{1}{\beta_{2k}^2}{\sqrt{\mu}}\right].\end{equation}
%If $x''$ is another stationary point of $\kfir$ then $\card(x'') > k$.
%\end{corollary}



Note that we allow $\delta_N^-<0$ in the above theorem, in which case the condition on $z'$ is automatically satisfied. The proof depends on a sequence of lemmas, and is given at the end of the section. Clearly, we will rely on Proposition \ref{thm:statpoint}, which requires an investigation of the functional $\G$ \eqref{gdef} and in particular its sub-differential. Introducing the function $g$ as
\begin{equation}
g(x) =
\begin{cases}
\frac{\mu + {x^2}}{2} & |x| \geq {\sqrt{\mu}} \\
\sqrt{\mu}|x| & 0 \leq |x| \leq {\sqrt{\mu}}
\end{cases}.
\label{eq:gdef}
\end{equation}
we get \begin{equation}\label{Gg}
\G(x)=\sum_{j=1}^n g(x_j).\end{equation}
Its sub-differential is given by
\begin{equation}
\partial g(x) =
\begin{cases}
\{ x\} & |x| \geq {\sqrt{\mu}} \\
\{\sqrt{\mu}\frac{x}{|x|}\} & 0 < |x| \leq {\sqrt{\mu}} \\
\sqrt{\mu}~\D & x = 0
\end{cases}
\label{eq:vectorsubgrad}
\end{equation} where $\D$ is the closed unit disc in $\C$ or, if working over $\R$, $\D=[-1,1]$. In the remainder we suppose for concreteness that we work over $\C$ (but show the real case in pictures).
Note that the sub-differential consists of a single point for each $x \neq 0$.
Figure~\ref{fig:gfunk} illustrates $g$ and its sub-differential.
\begin{figure}[htb]
\begin{center}
\includegraphics[width=40mm]{gfunk}
\includegraphics[width=40mm]{gsubgrad}
\end{center}
\caption{The function $g(x)$ (left) and its sub-differential $\partial g(x)$ (right). Note that the sub-differential contains a unique element everywhere except at $x=0$.}
\label{fig:gfunk}
\end{figure}

%Our goal is now to find constraints that assure that this system of equations have only one solution. Before getting into the details we outline the overall idea.
%For simplicity consider two differentiable strictly convex functions $\tilde{h}$ and $\tilde{g}$.
%Their sum is minimized by the stationary point $x_s$ fulfilling $- \nabla \tilde{h}(x_s) = \nabla \tilde{g}(x_s)$.
%Since $\tilde{g}$ is strictly convex its directional derivative $\nabla \tilde{g} (x_s + t \v)^T \v$ is increasing for all $\v \neq 0$.
%Similarly $-\nabla \tilde{h} (x_s + t \v)^T \v$ is decreasing for all $\v\neq 0$ since $-\tilde{h}$ is strictly concave. Therefore $-\nabla \tilde{h} (x_s + t \v)^T \v < \nabla \tilde{g} (x_s + t \v)^T \v$ which means that $x_s$ is the only stationary point.
%In what follows we will estimate the growth of the directional derivatives of the functions involved in \eqref{eq:vectorobj} in order to show a similar contradiction.
%For the function $h$ we do not have convexity, however due to \eqref{eq:vectorRIP} we shall see that it behaves essentially like a convex function for sparse vectors $x$. Additionally we have to consider the non-convex perturbation $-\delta \|x\|^2$. Therefore we need somewhat sharper estimates than just growth of the directional derivatives of $g$.


The following two results establish a bound on the sub-gradients of $\G$.  We begin with some one-dimensional estimates of $g$.
%Due to convexity of $g$ it is clear that at any point $x$ these are growing in all directions $\v$.
%However, in order to guarantee uniqueness of a sparse stationary point we need to show that they grow faster than $2\delta \|\v\|^2$.
%Loosely speaking we will show that provided that the vector $\frac{1}{2}z$, where $z \in \partial g (x)$ is the sub-gradient, has elements that are not too close to the thresholds $\pm \sqrt{\mu}$ this will be true.

\begin{lemma}\label{lemma:bnd1}
Assume that $z_0 \in \partial g(x_0)$ and $\delta_N^->0$.
If
\begin{equation}
\left|
z_0
\right| > \frac{\sqrt{\mu}}{1-\delta_N^-}
\label{eq:subgradbnd1}
\end{equation}
then for any $x_1,~z_1$ with $z_1\in \partial g(x_1)$ and $x_1\neq x_0$, we have
\begin{equation}\label{fd}
\re(z_1 -z_0)\overline{(x_1-x_0)} > \delta_N^- |x_1-x_0|^2 .
\end{equation}
\end{lemma}
\begin{proof}
By rotational symmetry (i.e. $\partial g(e^{i\phi}x)= e^{i\phi} \partial g(x)$), it is no restriction to assume that $z_0>0$. By $\frac{1}{1-\delta_N^-}> 1$ and \eqref{eq:subgradbnd1}, we see that $z_0>\sqrt{\mu}$, and hence the identity $z_0\in\partial g(x_0)$ and \eqref{eq:vectorsubgrad} together imply that $z_0=x_0$ and in particular that $x_0\in\R$ and
\begin{equation}
\label{onion}x_0>\frac{\sqrt{\mu}}{1-\delta_N^-}.
\end{equation}
To prove the result we now minimize the quotient
$\frac{\re(z_1 -z_0)\overline{(x_1-x_0)}}{ |x_1-x_0|^2}$ and show that it is larger than $\delta_N^-$.
There are three cases to consider; $|x_1|=0$, $0<|x_1|<\sqrt{\mu}$ and $|x_1|\geq \sqrt{\mu}$. The latter case is easy since then $z_1-z_0=x_1-x_0$ and $\delta_N^- < 1$, which yields the desired conclusion.

For the two other cases we first show that $z_1$ and $x_0$ can be assumed to be real.
If $x_1=0$ then the optimization of the above quotient is equivalent to minimization of $-\re(z_1)$ over $z_1 \in \sqrt{\mu}\D$, since $x_0=z_0$ is real and positive, which is clearly minimized in $z_1 = \sqrt{\mu}$.
For the middle case, $z_1$ and $x_1$ have the same angle with $\R$, and $|x_1|<|z_1|<z_0$. We first hold the radii fixed and only consider the angle as an argument. Recall $z_0=x_0$ and set $R=|z_1|/|x_1|$. Then we have 
 \[ \begin{split} \frac{\re(z_1 -z_0)\overline{(x_1-x_0)}}{ |x_1-x_0|^2} & =\frac{R|x_1|^2-2R\re x_1 \overline{x_0}+|x_0|^2}{ |x_1-x_0|^2} \\ & = \frac{R(|x_1|^2-2\re x_1 \overline{x_0}+|x_0|^2) - R |x_0|^2 + |x_0|^2}{|x_1-x_0|^2}  \end{split}  \] that equals \begin{equation}\label{gt}R- \frac{R-1}{|x_1-x_0|^2} |x_0|^2 \end{equation}
which shows that the quotient is minimized when $x_1$ is real and $0<x_1<\sqrt{\mu}$ (which then automatically applies to $z_1$ as well).

Summarizing the above we may thus assume that $x_1$ and $z_1$ are real and non-negative and $0\leq x_1<\sqrt{\mu}$. This simplifies the quotient \eqref{gt} to $\frac{x_0-z_1}{ x_0-x_1}$. We now hold $x_1,~z_1$ fixed and consider $x_0$ as the variable. Since $z_1\geq x_1$, it is easy to see that this is minimized for $x_0$ as small as possible, i.e. $x_0=\frac{\sqrt{\mu}}{1-\delta_N^-}$. With this at hand, the minimum of $\frac{|z_1-\frac{\sqrt{\mu}}{1-\delta_N^-}|}{ |x_1-\frac{\sqrt{\mu}}{1-\delta_N^-}|}$ is clearly attained at $x_1=0$ and $z_1=\sqrt{\mu}$. Summing up, we have that
$$\frac{\re(z_1 -z_0)\overline{(x_1-x_0)}}{ |x_1-x_0|^2}>\frac{|z_1-\frac{\sqrt{\mu}}{1-\delta_N^-}|}{ |x_1-\frac{\sqrt{\mu}}{1-\delta_N^-}|}\geq \frac{|\sqrt{\mu}-\frac{\sqrt{\mu}}{1-\delta_N^-}|}{ |\frac{\sqrt{\mu}}{1-\delta_N^-}|}=\delta_N^-.$$
\end{proof}

\begin{lemma}\label{lemma:bnd2}

Assume that $z_0 \in \partial g(x_0)$ and $\delta_N^->0$.
If
\begin{equation}
\left|
z_0
\right| < {(1-\delta_N^-)}{\sqrt{\mu}}
\label{eq:subgradbnd2}
\end{equation}
then for any $x_1,~z_1$ with $z_1\in \partial g(x_1)$, $x_1\neq x_0$, we have
\begin{equation}\label{fd1}
\re(z_1 -z_0)\overline{(x_1-x_0)} > \delta_N^- |x_1-x_0|^2.
\end{equation}\end{lemma}
\begin{proof}
The proof is similar to the previous lemma. We first note that $x_0=0$, $x_1\neq 0$ and that $z_0$ may be assumed to be in $(0,\sqrt{\mu}]$. For a fixed radius $R = \frac{|z_1|}{|x_1|}$ the quotient \[\frac{\re(z_1 -z_0)\overline{(x_1-x_0)}}{ |x_1-x_0|^2}=\frac{\re(z_1 -z_0)\overline{x_1}}{ |x_1|^2} = R- z_0\frac{\re  x_1}{|x_1|^2} \] is smallest when both $x_1$ and $z_1$ are real valued and positive.
Since $x_1\neq 0$ we have $z_1 = \max(x_1,\sqrt{\mu})$.
Clearly $z_0={(1-\delta_N^-)}{\sqrt{\mu}}$ gives a minimum value for any positive choice of $x_1,z_1$, because \( |z_0 \re (x_1) / |x_1|^2 | < {(1-\delta_N^-)}{\sqrt{\mu}} | \re (x_1) / |x_1|^2 |   \).
This reduces the problem to finding the minimum of $$x_1 \mapsto\frac{\max(x_1,\sqrt{\mu}) -{(1-\delta_N^-)}{\sqrt{\mu}}}{ x_1}$$ which by basic calculus equals $\delta_N^-,$ as desired.
\end{proof}


We are now ready to prove Theorem \ref{thm:statpoint:vec}.

\begin{proof}[Proof of Theorem \ref{thm:statpoint:vec}]
By Proposition \ref{thm:statpoint} it suffices to verify \begin{equation}\label{g}
\re\skal{z''-z',x''-x'} > \delta_N^- \|x''-x'\|_2^2,\quad x''\neq x'.
\end{equation} The claim will follow by contradiction.
Suppose first that $\delta_N^->0$. Since $\partial \G(x)=\sum_{j=1}^n \partial g(x_j)$, Lemmas \ref{lemma:bnd1} and \ref{lemma:bnd2} imply that
$$\re(z''_i-z'_i) \overline{(x_i''-x_i')} > \delta_N^- |x_i''-x_i'|^2,
$$
for all $i$ with $x_i''-x_i' \neq 0$. Since $x_i''-x_i'=0$ gives $(z''_i-z'_i)\overline{(x_i''-x'_i)}=0$
summing over $i$ gives the result.


Suppose now that $\delta_N^->1$. By \eqref{g} it suffices to prove that $\re\skal{z''-z',x''-x'}\geq 0$ for all $x''\neq x'$. Fix $i$ in $\{1,\ldots,n\}$. By rotational symmetry it is easy to see that we can assume that $x'_i,z'_i\geq 0$. Moreover, for fixed values of $|z_i''|$ and $|x''_i|$ (but variable complex phase) it is easy to see that $\re (z_i''-z')(x_i''-x_i')$ achieves min when these are also real, i.e. we can assume that $x''_i,z''_i\in\R$. Since the graph of $\partial g$ is non-decreasing it follows that $(z_i''-z')(x_i''-x_i') \geq 0$ for all $i$, as desired.

It remains to consider the case when $\delta_N^-=1$, and as above we reach a contradiction if we prove that $\re\skal{z''-z',x''-x'}> 0$. Again we can assume that $x'_i,z'_i\geq 0$ and that $x''_i,z''_i\in\R$. Then \eqref{e4} implies that $z_i'\neq \sqrt{\mu}$ for all $1\leq i \leq n$, which via $z'_i\in \partial g(x'_i)$ also implies that $x_i'\not\in (0,\sqrt{\mu}]$. If $x''\neq x'$ we must have $x''_i\neq x_i$ for some $i$. Using that $z_i''\in \partial g$, examination of \eqref{eq:vectorsubgrad} yields that also $z_i''\neq z_i'$.
With this at hand we see that the left hand side of \eqref{g} is strictly positive, whereas the right equals 0, which again is a contradiction.

\end{proof}

\iffalse
For later use in [..], we record that we have shown the following result. \begin{corollary}\label{corbor}
Let $z'$ satisfy $z'\in\partial \G(x')$ and
\begin{equation}\label{e4t}|z_i'|\not\in\left[{\lambda^2}{\sqrt{\mu}},\frac{1}{\lambda^2}{\sqrt{\mu}}\right].\end{equation}
If $z''\in\partial \G(x'')$, then $\re\scal{z''-z',x''-x'}>(1-\lambda^2)\|x''-x'\|_2^2$.
\end{corollary}
\fi

\subsection{Conditions on global minimality}\label{erai1}

\begin{theorem}\label{thm:globalpoint2}
Let $A$ satisfy $\|A\|_{\infty,col}\leq 1$, let $x'$ be a stationary point of $\kfir$ and let $z'$ be given by \eqref{y}. Assume that
\begin{equation}\label{cond3}|z_i'|\not\in\left[{(1-\delta_N^-)}{\sqrt{\mu}},\frac{1}{1-\delta_N^-}{\sqrt{\mu}}\right],\quad 1\leq i\leq n.\end{equation}
If \begin{equation}\label{cond2}2\mu\card(x') +\fro{Ax'-b}< \mu N+\mu,\end{equation} then $x'$ is the unique global minimum of $\kfi$ and $\kfir$.
\end{theorem}

Obviously, it is desirable to pick $N$ as large as possible, which is limited by \eqref{cond3} and the fact that $\delta_N^-$ increases with $N$. Also note that $\delta_N^-\geq 0$ since $1-\delta_1^-\leq \sup_i\{\|a_i\|_2^2\}=\|A\|_{\infty,col}^2\leq 1$.

\begin{proof}
Set $k=\card(x')$ and assume that $x'$ is not the unique global minimizer of $\kfir$.
By Theorem \ref{celok5}, there exists a global minima $x''\neq x'$ for both $\kfir$ and $\kfi$, which hence is a stationary point of $\kfir$. Theorem \ref{thm:statpoint:vec} then shows that $\card (x'')\geq N-k+1$. It follows that
$$\kfir(x'')-\kfir(x')\geq \kfi(x'')-\kfi(x')\geq \mu(N-k+1)-(\mu k +\fro{Ax'-b})>0$$
by \eqref{cond2}, $\kfi(x'')=\kfir(x'')$ and $\kfi(x')\geq\kfir(x')$. This is a contradiction, and hence $x'$ must be the unique global minimizer of $\kfir$. By Theorem \ref{celok5} it then follows that $x'$ is also unique minimizer of $\kfi$.
\end{proof}




\subsection{Noisy data.}
In this final subsection we return to the compressed sensing problem of retrieving a sparse vector $x_0$ given corrupted measurements $b=Ax_0+\ep$, where $\ep$ is noise and $x_0$ is sparse. More precisely we set $S=\supp x_0$ where we assume that $\#S=k$ is much smaller than $m$ -- the amount of rows in $A$ (i.e. number of measurements). We let $x_{0,j}$ denote the elements of the vector $x_0$. Let $A_S$ denote the matrix obtained from $A$ by setting columns outside of $S$ to $0$, and let $x_S$ denote the least squares solution to $A_S x_S=b$. Note that this is the so called ``oracle solution'' discussed in the introduction, which can also be written $x_S=(A_S^*A_S)^\dagger A_S^*b$ where $(A_S^*A_S)^\dagger$ denotes the Moore-Penrose inverse. The below proposition shows that the oracle solution is under mild assumptions a local minimizer of $\K_{reg}$, which we denote by $x'$ for notational consistency.

\begin{proposition}\label{p1}
Let $A$ satisfy $\|A\|_{\infty,col}\leq 1$. If $\|\ep\|_2< {\sqrt{\mu}}$ and $$|x_{0,j}|>\sqrt{\mu}+\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}$$ for all $j\in S$ then the oracle solution $x'=x_S$ is a strict local minimum to $\kfir$ with $\supp (x')=\supp (x_0)$. We also have $|x_{j}'|>\sqrt{\mu},~ j\in S,$ $\|Ax'-b\|_2\leq \|\epsilon\|_2$, and $$\|x'-x_0\|_2\leq \frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}.$$
\end{proposition}
%do we need to prove this or showing stationary point is enough??????????
\begin{proof}
Consider the equation $A_Sx=Ax_0+\ep$ and note that $Ax_0=A_Sx_0$. The least squares solution is obtained by applying $(A_S^*A_S)^\dagger A_S^*$ which gives the solution $$x'=x_0+(A_S^*A_S)^\dagger A_S^*\ep=x_0+\eta,$$ where we set $(A_S^*A_S)^\dagger A_S^*\ep=\eta$. By construction of the Moore-Penrose inverse, $\supp \eta\subset S$, and hence $$A\eta=A_S\eta=P_{\text{Ran} A_S}\ep,$$ where $P_{\text{Ran} A_S}$ denotes the orthogonal projection onto the range of $A_S.$ In particular, $$\|\eta \|_2\leq\frac{\|A_S\eta\|_2}{\sqrt{1-\delta_k^-}}=\frac{\|P_{\text{Ran} A_S}\ep\|_2}{\sqrt{1-\delta_k^-}}\leq \frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}},$$
which establishes the final inequality in the proposition. Also $\|\eta\|_{\infty}\leq \|\eta\|_{2}$ which implies \begin{equation}\label{sofg}|x_{j}'|\geq |x_{0,j}|-|\eta_j|>\sqrt{\mu}+\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}-\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}=\sqrt{\mu},\quad j\in S.\end{equation} This also gives $\supp x'=\supp x_0$ since by construction we clearly have \[\supp x' \subset \supp x_0\cup\supp \eta \subset S.\]

We now consider $Ax'-b$, which equals \begin{equation}\label{sof}\begin{aligned}&=A_Sx'-b\\&=A_Sx_0+A_S(A_S^*A_S)^\dagger A_S^*\ep-(A_Sx_0+\ep)\\&=(P_{\text{Ran} A_S}-I)\ep\\&=-P_{(\text{Ran} A_{S})^{\perp}}\ep\end{aligned}\end{equation}
and hence $\|Ax'-b\|_2\leq \|\epsilon\|_2$.

It remains to prove that $x'$ is a local minimum of $\kfir=\Q_2(\mu\card)+\fro{Ax-b}$. To this end, consider $\kfir(x'+v)$. Since $|x_{j}'|>\sqrt{\mu}$ for $j\in S$, the term $\Q_2(\mu\card)$ is flat for the corresponding indices of $v$. We get \begin{equation}\label{rd}\kfi(x'+v)=\sum_{j\in S^c}\left(2\sqrt{\mu} |v_j|-v_j^2\right)+2\scal{v,A^*(Ax'-b)}+\|Av\|_2^2+\kfir(x').\end{equation} Since $x'$ solves the least squares problem posed initially, the vector $A_S^*(Ax'-b)=A_S^*(A_Sx'-b)$ must be 0. With this in mind \eqref{rd} then simplifies to \begin{equation}\label{rd1}2\left(\sum_{j\in S^c}\sqrt{\mu} |v_j|+v_j\scal{a_j,Ax'-b}\right)-\sum_{j\in S^c}v_j^2+\|Av\|_2^2+\kfir(x').\end{equation} By the Cauchy-Schwartz inequality and \eqref{sof} we have $$|\scal{a_j,Ax'-b}|\leq \|a_j\|_2\|\ep\|_2< \|A\|_{\infty,col} {\sqrt{\mu}}\leq\sqrt{\mu}.$$ It follows that the term $\sum_{j\in S^c}\sqrt{\mu} |v_j|+v_j\scal{a_j,Ax'-b}$ in \eqref{rd1} can be estimated from below as follows: \[  > \sum_{j \in S^c}  |v_j|( \underbrace{\sqrt{\mu} + \min\{ 0,\text{sign}(v_j) \langle a_j, A x' - b \rangle\}}_{:= \alpha_j}   ) \ge \rho\sqrt{\sum_{j\in S^c}v_j^2}     \]for some $\rho>0$, where \( \alpha_j > 0  \) for all \(j\) and we used the equivalence between \( \ell^1 \) and \( \ell^2  \) norms. Hence $$2\left(\sum_{j\in S^c}\sqrt{\mu} |v_j|+v_j\scal{a_j,Ax'-b}\right)-\sum_{j\in S^c}v_j^2>0$$ for $v$ in a neighborhood of 0, as long as $\sum_{j\in S^c}v_j^2\neq 0$. To have $\kfir(x'+v)\leq\kfir(x')$ we thus need $\supp v\subset S$, as seen from \eqref{rd1} (and this because both summations in \eqref{rd1} are over \( S^c \), but if $\supp v\subset S$ then \( v_j = 0  \) for all \( j \in S^c \)). But then \eqref{rd1} reduces to $\|Av\|_2^2+\kfir(x')$, and since ${\delta_k^-}<1$ it follows that $\|Av\|_2^2>0$ unless $v=0$. In other words, $x'$ is a strict local minimizer.
\end{proof}

%By the above proof, an explicit formula for $x_1$ is
%\begin{equation}\label{ko}x_1=x_0+(A_S^*A_S)^\dagger A_S^*\ep.\end{equation}

In the above proposition, there is nothing said as to whether $x'$ is a global minimum or not. To get further, let $z'$ correspond to $x'$ via \eqref{y}. We need conditions such that \eqref{cond3} holds for $z'$, i.e.
\begin{equation}\label{cond31}|z_{i}'|\not\in\left[{(1-\delta_N^-)}{\sqrt{\mu}},\frac{{\sqrt{\mu}}}{1-\delta_N^-}\right].\end{equation}
We remind the reader that $N$ is a number which preferably is a bit larger than $2k$, where $k$ is the cardinality of $x_0$.



\begin{proposition}\label{p2}
Let $A$ satisfy $\|A\|_{\infty,col}\leq 1$. If $\|\ep\|_2< {(1-\delta_N^-)\sqrt{\mu}}$ and \begin{equation}\label{po7}|x_{0,j}|>\frac{\sqrt{\mu}}{1-\delta_N^-}+\frac{(1-\delta_N^-)\sqrt{\mu}}{\sqrt{1-\delta_k^-}}, \quad j\in \supp x_0,\end{equation}
then \eqref{cond31} holds.
\end{proposition}
\begin{proof}
Using \eqref{sof} we get
\begin{align}\label{tg}z'=( I-A^* A)x' + A^* b =  x'-A^*(Ax'-b)= x'+A^*P_{(\text{Ran} A_{S})^{\perp}}\ep.\end{align}
Since $A^*P_{(\text{Ran} A_{S})^{\perp}}$ is 0 on rows with index $j\in S$ (being a scalar product of a vector in $\text{Ran} A_{S}$ and another in its orthogonal complement), we see that $z_{j}'= x_{j}'$ for such $j$. Combining this with the final estimate of Proposition \ref{p1}, we see that  \begin{equation*}\label{po9}|z_{j}'|>\frac{1}{1-\delta_N^-}{\sqrt{\mu}}, \quad j\in S\end{equation*} holds whenever \begin{equation}\label{po6}|x_{0,j}|>\frac{\sqrt{\mu}}{1-\delta_N^-}+\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}, \quad j\in S,\end{equation} which is true by the assumptions. For the remaining $z_{j}'$, (i.e. $j\in S^c$), we have $x_{j}'=0$ so \begin{equation}\label{o0}\begin{aligned}&|z_j'|=|(A^*P_{(\text{Ran} A_{S})^{\perp}}\ep)_j|=|\scal{P_{(\text{Ran} A_{S})^{\perp}}\ep,a_j}|\leq \\&\|A\|_{\infty,col}\|\ep\|_2\leq \|\ep\|_2<{(1-\delta_N^-)}{\sqrt{\mu}},\end{aligned}\end{equation}
which establishes \eqref{cond31}.
\end{proof}


Putting all the results together and combining with simple estimates, we finally get

\begin{theorem}\label{thm:doctorgadget}
Suppose that $b=Ax_0+\ep$ where $A$ is an $m\times n$-matrix with $\|A\|_{\infty,col}\leq 1$ and set $\card (x_0)=k.$ Let $N\geq 2k$ and assume that
$\|\ep\|_2< {(1-\delta_N^-)\sqrt{\mu}}$ and $$|x_{0,j}|>\para{\frac{1}{1-\delta_N^-}+1}\sqrt{\mu},\quad j\in \supp x_0.$$ Then the oracle solution $x'=x_S$ is a unique global minimum to $\kfir$ as well as $\kfi$, with the property that $\supp x'=\supp x_0$, that $$\|x'-x_0\|_2\leq \frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}},$$ and that $\card(x'')> N-k$ for any other stationary point $x''$ of $\kfir$.
\end{theorem}

\iffalse
A necessary condition for the above assumptions to hold, is that they hold with $\beta_{N}$ replaced by $\sigma_{N}$, in light of Proposition \ref{p0}.
\fi
\begin{proof}
All the statements follow by Theorem \ref{thm:statpoint:vec}, Theorem \ref{thm:globalpoint2} and Proposition \ref{p1}, so we just need to check that these apply. Note that $\sqrt{1-\delta_{N}^-}\leq \sqrt{1-\delta_k^-}\leq \|A\|_{\infty,col}\leq 1$ which will be used repeatedly.


We begin to verify that Proposition \ref{p1} applies, which is easy by noting that $\|\ep\|_2\leq (1-\delta_N^-)\sqrt{\mu}<2\sqrt{\mu}$ and $${\sqrt{\mu}}+\frac{\|\epsilon\|_2}{\sqrt{1-\delta_k^-}}\leq \frac{\sqrt{\mu}}{1-\delta_N^-}+\frac{(1-\delta_N^-)\sqrt{\mu}}{\sqrt{1-\delta_k^-}}\leq \frac{\sqrt{\mu}}{1-\delta_N^-}+{\sqrt{\mu}}<|x_{0,j}|.$$

Now, to verify that the two theorems apply we need to check the conditions \eqref{cond31}, which follow if we show that Proposition \ref{p2} applies. The estimate on $\|\ep\|_2$ is satisfied by assumption and the other follows by noting that $\frac{1-\delta_N^-}{\sqrt{1-\delta_k^-}}\leq 1.$ By this we already have verified Theorem \ref{thm:statpoint:vec} and the first condition of Theorem \ref{thm:globalpoint2}. To check  \eqref{cond2} note that $\|Ax'-b\|_2\leq \|\ep\|_2< (1-\delta_N^-)\sqrt{\mu}$ by Proposition \ref{p1}, so \eqref{cond2} holds if $2\mu k+(1-\delta_N^-)^2{\mu}\leq \mu N+\mu$, which is clearly the case since $N\geq 2k$.

\end{proof}

As usual, a simpler statement is found by setting $N=2k$, which gives the loosest conditions to verify, (see Corollary \ref{cor:doctorgadget}). The only difference in the conclusion concerns the cardinality of other local minima, since the estimate on $\|x'-x_0\|_2$ only depends on $\delta_k^-$.



\section{Known model order; the $k$-sparsity problem}\label{seccardfix}

Let $P_k=\{x:\card (x)\leq k\}$ where $x$ is a vector in $\C^n$ or $\R^n$. Set $f(x)=\iota_{P_k}(x)$ and note that the problem \begin{equation}\label{agt1}\argmin_{\card(x)\leq k}\|Ax-b\|_2\end{equation} is equivalent to finding the minimum of \begin{equation}\label{agt2}\ksi(x)=\iota_{P_k}(x)+\|Ax-b\|_2^2,\end{equation}
(where we put a subindex $k$ to distinguish from $\K$ in the previous section). Again, we will approach this problem by using
$$\ksir(x)=\Q_2(\iota_{P_k})(x)+\|Ax-b\|_2^2.$$
This is in some ways much simpler than the situation in the previous sections, for example all local minimizers of $\ksi$ are clearly in $P_k$.
On the other hand, $\Q_2(\iota_{P_k})$ turns out to be rather complicated. We recapitulate the essentials, which follows by adapting the computations in \cite{andersson-etal-ol-2017} (for matrices) to the vector setting. Define $\tilde x$ to be the vector $x$ resorted so that $(|\tilde x_j|)_{j=1}^d$ is a decreasing sequence. Then
%\begin{equation}\label{lust2}\S(\iota_{P_k})(y)= \sum_{j=k+1}^d -|\tilde y_j|^2\end{equation}
\begin{equation}\label{lust1}\Q_2(\iota_{P_k})(x)= \frac{1}{k_*}\para{\sum_{j>k-k_*}|\tilde{x}_j|}^2-\sum_{j>k-k_*}|\tilde x_j|^2\end{equation} where $k_*$ is the largest value of \(l \in \{1,\dots,k\} \) for which the non-increasing sequence
\begin{equation}\label{lust}s(l)=\left(\sum_{j>k-l}|\tilde x_j|\right)-l|\tilde x_{k+1-l}|\end{equation}
is non-negative (note that it clearly is non-negative for $l=1$); finding \( k_* \) has complexity (at worst) \( O(d^2) \). Although it is not very clear from the above expression, $\Q_2(\iota_{P_k})$ is known to be continuous (see e.g.~Proposition 3.2 in \cite{carlsson2018convex}), and this will be used without comment below. We first show that the global minima of $\ksir$ and $\ksi$ coincide.

\subsection{Equality of minimizers and $k$-feasibility}\label{Kfeas}

In order to provide a theorem similar to \ref{celok5}, we need a technical condition on the columns $a_1,\ldots,a_n$ of $A$. We say that $A$ is \textit{$k$-feasible} if $\|A\|_{\infty,col}\leq 1$ and for any subset of $n-k$ columns, we can pick two such that $\|a_i-a_j\|_2^2\leq 2$. We say that $A$ is \textit{strictly $k$-feasible} if the inequality is strict. This is very easy to satisfy, the following proposition lists conditions that imply $k$-feasibility in $\R$ and $\C$ respectively.
\begin{proposition}\label{mfisR}
If we work over $\R$, any $A$ with $\|A\|_{\infty,col}\leq 1$ and $n\geq m+k+2$ is $k-$feasible. If we add the condition that $\scal{a_i,a_j}\neq 0$ for all pairs, or that $\|A\|_{\infty,col}< 1$, then strict $k-$feasibility follows. The same follows over $\C$ if $n\geq 2m+k+2$. Another condition ensuring strict $k-$feasibility, which works in both $\R$ and $\C$, is that $\|A\|_{\infty,col}\leq 1$ and at least $nk$ of the values $\{\re\scal{a_i,a_j}\}_{i> j}$ are positive (repetitions allowed).
\end{proposition}
We remark that it is possible to choose $2m+1$ vectors in $\C^m$ such that $\|a_i-a_j\|_2^2> 2$, just consider a simplex in $\R^{2m}$ with equal sidelengths and all corners on the unit sphere. The condition that $n\geq 2m+k+2$ is a bit unfortunate, since it rules out the common situation $n=2m$. This is why we added the final part of the proposition.

\begin{proof}
If the chosen subset contain a zero vector, the conclusion is immediate, so we can assume that this is not the case. For any $m+2$ vectors $a_1,\ldots,a_{m+2}$ in $\R^m$, we can always pick two such that $\scal{a_i,a_j}\geq 0$, which follows from a simple induction argument: this is indeed clear in \( \mathbb{R} \); in \( \mathbb{R}^{m} \) take \( m+2 \) vectors \( v_i\) such that \( \langle v_i , v_j \rangle < 0  \) if \( i \ne j  \). If \(V\) is the orthogonal to \( v_{m+2}  \), the projections of \( v_1, \dots , v_{m+1} \) on \( V  \) have the same property, and \( V\) is an \((m-1)\)-dimensional vector space. By induction we would get the same conclusion for \( \mathbb{R}  \), which is a contradiction.

The first two conclusions regarding $\R^m$ follow immediately by this observation. Since $\C^m$ is isomorphic with $\R^{2m}$, the corresponding result for $\C$ follows. Finally, the elements above the diagonal in $(\scal{a_i,a_j})_{i,j=1}^n$ are $n(n-1)/2$ in number. When we consider a subset of columns of cardinality $n-k$, we remove a total of $(n-k)k+(k-1)k/2$ of these. Since $nk$ is a bigger number, we are certain that at least one positive value remain.
\end{proof}


To illustrate a concrete example, which sometimes appears in applications, we consider the concatenation of a discrete Fourier transform matrix and an identity matrix. To see what the above proposition entails in this case, suppose that $m=4M$ or $m=4M+1$. Each column of the Fourier matrix gives rise to at least $M$ positive values in its scalar products with the canonical basis coming from the identity matrix, so in total we have at least $mM$ positive off diagonal elements in the Fourier matrix. This gives the condition $2mk\leq mM$, i.e.~$K\leq m/8$, which is acceptable for relevant applications. We now develop some theory for $k$-feasible matrices, starting with the analog of Theorem \ref{celok5}.




\begin{theorem}\label{celok6}
Let $A$ be $k$-feasible. Then the global minimizers of $\ksir$ and $\ksi$ coincides, and all lie in $P_k$. If $A$ is strictly $k$ feasible, then any local minimizer of $\ksir$ lies in $P_k$ and is a minimizer of $\ksi$.
\end{theorem}

\begin{proof} We first treat global minimizers. Clearly all minimizers of $\ksi$ are in $P_k$. Since $\ksi\geq\ksir$ and they coincide on $P_k$, it suffices to show that a given global minimizer of $\ksir$ is in $P_k$. This is annoyingly difficult, it is even a problem to show that $\ksir$ has global minima. We begin by showing that large values of $x$ are not candidates for global minima if they are in the set $$U=\left\{x\neq 0:~\frac{\sum_{j=k+1}^n|\tilde x_j|}{\sum_{j=1}^k|\tilde x_j|}\geq\frac{1}{2k}\right\}.$$ We have $\Q_2(\iota_{P_k})(x)>0$ for all $x\in U$. One way to see this is by Corollary 4.4 in \cite{carlsson2018convex} (or Theorem 2.20 in \cite{carlsson2016convexification}), which states that there exists a direction $v$ such that $t\mapsto \Q_2(\iota_{P_k})(x+tv)>0$ has negative second derivative (since $\ksir(x)<\infty=\ksi(x)$), and this would imply that $\Q_2(\iota_{P_k})$ could take negative values, contradicting Proposition 3.2 in \cite{carlsson2018convex} (or Proposition 2.1 in \cite{carlsson2016convexification}). This can also be deduced by a more careful analysis of \eqref{lust1}, which we will perform below. Define \begin{equation}\label{olbia}\alpha =\inf\left\{\Q_2(\iota_{P_k})(x): ~x\in U,~\|x\|_2=1\right\}.\end{equation}
Since we are minimizing a continuous non-zero function over a compact set, $\alpha>0$. We now show that large values of $x\in U$ yield large values of $\Q_2(\iota_{P_k})(x)$. Let us write $s=s_x$ for \eqref{lust}, when there is a need to make the dependence on $x$ clear. The function $s$ is radially dependent, i.e.~$s_{tx}=t s_x$ for $t\in\R$, and hence $k_*$ is radially independent. Looking at the expression for $\Q_2(\iota_{P_k})$ we see that $$\Q_2(\iota_{P_k})(tx)=t^2\Q_2(\iota_{P_k})(x)\quad t\in \R.$$
Note that $\ksi(0)=\ksir(0)=\frac{1}{2}\|b\|_2^2$ so the global minimum is less than or equal to this. If $R$ is such that $\alpha R^2>\frac{1}{2}\|b\|_2^2$, it finally follows that no point $x\in U$ with $\|x\|_2>R$ can be less than $\frac{1}{2}\|b\|_2^2$.

We remark in passing that $x=0$ can not be a global minimizer of $\ksir$ unless $b$ is perpendicular to the range of $A$, in which case the theorem holds trivially. To see this, note that
$\Q_2(\iota_{P_k})(0)=0$ and $\Q_2(\iota_{P_k})\geq 0$, so if $x=0$ is the global minimum of $\ksir$ the gradient of $\frac{1}{2}\|Ax-b\|_2^2$ must necessarily be zero at $x=0$, i.e.~$A^*(-b)=0$.


Now let $G$ be the set of global minimizers for $\ksir$ restricted to $[-R,R]^n$. This set is clearly closed, non-void and bounded. Now let $G_n\subset G$ be the subset where $|\tilde x_n|$ attains its minimum over $G$, let $G_{n-1}\subset G_n$ be the subset where $|\tilde x_{n-1}|$ is minimized, and so on until we reach $G_{k+1}$, which still is closed, non-void and bounded. Suppose that $G_{k+1}\not\subset P_k$ and pick $x\in G_{k+1}\setminus P_k$. We now show that this is impossible. First of all, note that any two columns of $A$ and corresponding two elements in $x$ may (simultaneously) switch positions and sign, without affecting the problem, so it is no restriction to assume that $|\tilde x|=x$ (i.e. \( x_i \ge 0 \) and \( x_i \ge x_{i+1} \) for all \(i\)), which we now do.

If $x_{k+1}=R$ then this must also be the case for $x_1,\ldots,x_k$, and hence $\|x\|_2>R$ and $x\in U$, which is impossible by the earlier conclusions. Thus $x_{k+1}<R$.

Use $k$-feasibility of $A$ to pick two indices $j>i> k$ such that $\|a_i-a_j\|_2^2\leq 2$. Consider the function \begin{equation}\label{function}x(t)=x+t e_i-te_j.\end{equation} We shall show that this function stays in $G$ for small values of $t>0$, which contradicts the construction of $G_{k+1}$. Note that it stays in $[-R,R]^n$ for sure, due to $x_{k+1}<R$.

A complicating factor is the fact that we may fail to have $|\tilde x(t)|=x(t)$ for $t>0$, i.e.~this vector is not necessarily non-increasing as a function of its index. As long as $ x_{k}> x_{i}$, we can pick both $i,j>k$ such that $x(t)$ is non-increasing for small values of $t>0$. We consider this case first. All values of $s_{x(t)}(l)$ in \eqref{lust} are then unaltered by $t$, and hence small perturbations do not affect $k_*$. With this at hand, it follows that the first term in the expression \eqref{lust1} for $\Q_2(\iota_{P_k})(x(t))$ is unaffected by small changes in $t$, whereas the latter term is a quadratic polynomial starting with $-2t^2$. The quadratic term in the expression $\|Ax(t)-b\|_2^2$ on the other hand is $\|a_i-a_j\|_2^2t^2$. Using $\|A\|_{\infty,col}\leq 1$, it follows that \begin{equation}\label{po0}\frac{d^2}{dt^2}\ksir(x(t))=-4+2\|a_i-a_j\|_2^2\leq 0.\end{equation} Thus $\ksir(x(t))$ is linear in a neighborhood of 0, and since $x(0)\in G$ it must actually be a constant. It follows that $x(t)\in G$ for small values of $t>0$, which is a contradiction as we noted before.

It remains to consider the case when $x_{k}= x_{i}$. In this case we can make $x(t)$ non-increasing (of its index) for small (fixed) values of $t>0$, upon changing $i$ so that $x_i$ is the first value to equal $x_k$, but now $i\leq l$ and the independence of $k_*$ is less clear. Let $k_i$ be such that $i=k+1-k_i$. We will need the following observations about $s(l)$; If $x_{k+1-l}=x_{k+1-(l+1)}$ then $s(l)=s(l+1)$ so we always have \begin{equation}\label{inh}x_{k+1-k_*}<x_{k+1-(k_*+1)}=x_{k-k_*}.\end{equation} Since $x\not \in P_k$, we also have $s_x(1)>0$. Combined this gives $s_x(k_i)=s_x(1)>0$ and hence $k_*\geq k_i$. If we now consider $s_{x(t)}(l)$ as functions of $t$, the inequality $s_{x(t)}(k_i)>0$ is stable with respect to small perturbations. On the other hand, the values of $s_{x(t)}(l)$ for $l>k_i$ are unaffected by small values of $t$ (they cancel out in the sum of \eqref{lust}), and so we conclude that $k_*$ is unaffected by small values of $t$. It follows that both terms depending on $t$ in $ x(t)$ have indices beyond $k-k_*$, which precisely as before yields that \eqref{po0} holds, a contradiction.

To sum up, we have so far shown that any element $x\in G_{k+1}\setminus P_k$ necessarily satisfies $|\tilde x_{k+1}|<R$ and $|\tilde x_n|=0$. As grande finale we will now show that this is impossible. Let $j$ be such that $x_j=0$ and pick $i$ such that $|x_i|\leq |{x}_k|$ and $\scal{a_i,a_j}\neq 0$. That this can be done follows from the basic fact that $m+1$ non-zero vectors in $\R^m$ can not be mutually orthogonal (suppose for the moment that no $a_i$ is identically 0). Since $x_j=0$, it is no restriction to assume that $\scal{a_i,a_j}> 0$, which we do for simplicity. Consider again $x(t)=x+t e_i- te_j$. The previous analysis can now be repeated without modification, to conclude that \eqref{po0} holds whether $i>k$ or not. But in this case \eqref{po0} has a strictly negative value, which contradicts that $x$ is in $G$ to begin with. In the case when one $a_i=0$, we have $\|a_i-a_j\|_2\leq 1$ for any other $a_j$, which also yields a contradiction in \eqref{po0}.

We can finally conclude that any minimizer of $\ksir$ in $[-R,R]^n$ is in $P_k$ and thus also a minimizer of $\ksi$. Since $R$ could be arbitrarily large, the conclusion holds also in $\R^n$. The set of global minimizers of $\ksir$ is thus closed and non-empty. However, the remaining argument becomes easier if we keep $R$ fixed where it is for a while longer.

Now consider a path-connected component $H$ of the set of global minimizers in $[-R,R]^n$. Repeating the entire above argument, we see that $P_k\cap H\neq\emptyset$. Assume now that it contains points that are not in $P_k$. Since $\sum_{j=l+1}^n |\tilde x_j|$ is a continuous function on $H$ which is 0 at $P_k$, there are points in $H$ with arbitrarily small quotient $(\sum_{j=l+1}^n|\tilde x_j|)/{|\tilde x_1|}$. Recall that we have ruled out the case $0\in H$ early on in the proof, so the quotient is a continuous function on $H$. Let $I$ be a level set of this function. We repeat the construction of sets $I_n\supset I_{n-1}\supset \ldots I_{k+1}$ precisely as we did with $G$. Pick a concrete $x\in I_{k+1}$, and as before it is no restriction to assume that $x=|\tilde x|$. As before we see that it is impossible to have $ x_n=0$, and as before we can pick $i,j$ such that $\scal{a_i,a_j}\geq 0$ where $i,j>k$. We define $x(t)$ via \eqref{function} and establish as before that the \eqref{po0} must hold, whereby we get that $x(t)\in I_{k+1}$ for small values of $t$, and this contradicts how the sets $I_1,\ldots, I_k$ were chosen.

By this we get that all global minimizers of $\ksir$ in $[-R,R]^n$ must lie in $P_k$, and since $R$ can be arbitrarily large, the proof about global minimizers is complete.

Finally if we assume that $A$ is strictly $k$-feasible and that $x$ is a local minimizer, then we can always find $i,j$ such that \eqref{po0} holds, which is a contradiction since  $-4+2\|a_i-a_j\|_2^2<0$ in this case.

\end{proof}



%If $\scal{a_i,a_j}\neq 0$ for all $i,j$ or if $\|A\|_{\infty,col}\leq 1$ then the above proof is easily modified to show that any local minimizer of $\ksir$ lies in $P_k$ and is a local minimizer also for $\ksi$. We omit the details.



\subsection{On the uniqueness of sparse stationary points}

We now give a condition, similar to \eqref{e4} in Section \ref{erai}, to ensure that a sparse stationary point is unique, in the sense that other stationary points must have higher cardinality.

\begin{theorem}\label{thm:statpoint:vecfix}
Let $x'$ be a stationary point of $\ksir$ with cardinality $k$, let $z'$ be given by \eqref{y}, and assume that
\begin{equation}\label{e4fix}|\tilde z'_{k+1}|<(1-2\delta_{2k}^-)|\tilde z'_{k}|.\end{equation}
If $x''$ is another stationary point of $\ksir$ then $\card(x'') > k$.
\end{theorem}



Again, we allow $\delta_{2k}^-<0$ in the above theorem, in which case the condition on $z$ is automatically satisfied. We begin with a lemma. Recall $\G$ given by \eqref{gdef}, i.e.~$\frac{1}{2}\Q_2(\iota_{P_k})(x)+\frac{1}{2}\fro{x}$ in the present case. We need an expression for $\partial\G(x)$ for $x\in P_k$.

\begin{lemma}\label{sun}
If $x\in P_k$ then $z\in\partial\G(x)$ if and only if $\tilde z_j=\tilde x_j$ for $j=1,\ldots,k$ and $\tilde z_j\in |\tilde x_k|\D $ for $j>k$.
\end{lemma}
\begin{proof}
Since $\Q_2(\iota_{P_k})+\fro{x}$ is the l.s.c. convex envelope of $\iota_{P_k}+\fro{x}$, we have that $\G(x)=\frac{1}{2}\Q_2(\iota_{P_k})+\frac{1}{2}\fro{x}$ is the double Fenchel conjugate of $\frac{1}{2}\iota_{P_k}+\frac{1}{2}\fro{x}$. The Fenchel conjugate of the latter is easily computed to $$\G^*(y)=\frac{1}{2}\sum_{j=1}^k |\tilde y_j|^2.$$ By the well-known identity $z\in\partial \G(x)\Leftrightarrow x\in\partial \G^*(z)$ (see e.g. Proposition 16.9 in \cite{bauschke2017convex}) we have $z\in\partial\G(x)$ if and only if \begin{equation}\label{t6}z=\argmax_z \re\scal{x,z}-\frac{1}{2}\sum_{j=1}^k |\tilde z_j|^2.\end{equation}
By standard results on reordering of sequences (see e.g.~Ch.~1 in \cite{simon2005trace}), this implies that the reordering of $z$ to $\tilde z$ can be chosen identical to that of $x$, which implies that $\scal{x,z}=\scal{\tilde x,\tilde z}$. Combined with $\tilde{x}_j=0$ for $j>k$, we see that \eqref{t6} turns into \begin{equation}\label{t7}z=\frac{1}{2}\argmax_z-\sum_{j=1}^k |\tilde x_j-\tilde z_j|^2.\end{equation} The lemma now easily follows.
\end{proof}





\begin{proof}[Proof of Theorem \ref{thm:statpoint:vecfix}.]
If $\card (x'')\leq k$ we clearly have $x''-x'\in P_{2k}$ and both $z'$ and $z''$ have the structure stipulated in Lemma \ref{sun}. Let $I'=\supp x'$ and $I''=\supp x''$. Then $\re\scal{z''-z',x''-x'}$ can be written
\begin{equation}
\re\left(\sum_{\footnotesize
\begin{array}{c}
i \in I' \\
i \in I''\end{array}}
|x_i''-x_i'|^2 +
\sum_{\footnotesize
\begin{array}{c}
i \in I' \\
i \notin I''\end{array}}
(x_i'-z_i'')\overline{x_i'} +
\sum_{\footnotesize
\begin{array}{c}
i \notin I' \\
i \in I''\end{array}}
(x_i''-z_i')\overline{x_i''}\right).
\label{eq:sum1}
\end{equation}
As before we want to reach a contradiction to Proposition \ref{thm:statpoint}, i.e.~we want to prove $\re\scal{z''-z',x''-x'}>\delta_{2k}^-\|x''-x'\|_2^2$. Note that
\begin{equation}\label{gr2}
\|x''-x'\|_2^2=\sum_{\footnotesize
\begin{array}{c}
i \in I' \\
i \in I''\end{array}}
|x_i''-x_i'|^2 +
\sum_{\footnotesize
\begin{array}{c}
i \in I' \\
i \notin I''\end{array}}
|x_i'|^2 +
\sum_{\footnotesize
\begin{array}{c}
i \notin I' \\
i \in I''\end{array}}
|x_{i}''|^{2},
\end{equation}
that the first term in \eqref{eq:sum1} and \eqref{gr2} are the same, and that $\delta_{2k}^-<1$. Since the second and third sums have the same number of terms it suffices to show that
\begin{equation}
\re (x_i'-z_i'')\overline{x_i'} + (x_j''-z_j')\overline{x_j''} > \delta_{2k}^-(|x_i'|^2 + |x_j''|^{ 2}),
\label{eq:twoterms}
\end{equation}
for any pair $i\in I'$, $i\notin I''$ and $j \notin I'$, $j \in I''$. This in turn will follow upon showing that
$$|z_i''| |x_i'| + |z_j'| |x_j''| < (1-\delta_{2k}^-)(|x_i'|^2 + |x_j''|^{ 2}).$$
By Lemma \ref{sun} it is easy to see that $|z_i''|\leq |z_j''|=|x_j''|$ and by assumption we also have $|z_j'|< (1-2\delta_{2k}^-)| z'_{i}|=(1-2\delta_{2k}^-)| x'_{i}|$. Thus \begin{equation*}\begin{split}|z_i''| |x_i'| + |z_j'| |x_j''|  <  |x_j''||x_i'| + (1-2\delta_{2k}^-)| x'_{i}| |x_j''| & = 2(1-\delta_{2k}^-)| x'_{i}| |x_j''| \\ & \leq (1-\delta_{2k}^-)(|x_i'|^2 + |x_j''|^{ 2}),\end{split}\end{equation*}
as desired.
\end{proof}


\iffalse
For later use in [..], we record that we have shown the following result. \begin{corollary}\label{corbor1}
Let $z'$ satisfy $2z'\in\partial \G(x')$ and
\begin{equation*}|\tilde z'_{k+1}|<(2\lambda^2-1)|\tilde z'_{k}|.\end{equation*}
If $2z''\in\partial \G(x'')$, then $\re\scal{z''-z',x''-x'}>(1-\lambda^2)\|x''-x'\|_2^2$.
\end{corollary}
\fi



\subsection{Conditions on global minimality.}
The statements in this section are actually a bit stronger than the corresponding ones in Section  \ref{erai1}.

\begin{theorem}\label{thm:globalpoint2f}
Let $A$ be $k$-feasible and let $x'\in P_k$ be a stationary point of $\ksir$. Let $z'$ be given by \eqref{y} and assume that \eqref{e4fix} applies. Then $x'$ is a unique global minimizer of $\ksi$ and $\ksir$. If $A$ is strictly $k$-feasible, then there are no other local minimizers either.
\end{theorem}
\begin{proof}
By Theorem \ref{celok6} there exists $x''\in P_k$ which is a global minimizer for both $\ksi$ and $\ksir$. If $x'\neq x''$ this would contradict Theorem \ref{thm:statpoint:vecfix}. If in addition $A$ is strictly $k$-feasible, then Theorem \ref{celok6} says that any local minimizer is a stationary point in $P_k$, which is impossible by Theorem \ref{thm:statpoint:vecfix}.
\end{proof}


\subsection{Noisy data.}
We now assume that $b$ is of the form $Ax_0+\ep$ where $\ep$ is noise and $x_0$ is sparse. More precisely we set $S=\supp x_0$ where we assume that $\#S=k$.
Let $A_S$ denote the matrix obtained from $A$ by setting columns outside of $S$ to $0$. By minor modifications of the proof of Proposition \ref{p1} we obtain.

\begin{proposition}\label{p1f}
Let $A$ satisfy $\|A\|_{\infty,col}\leq 1$. If $|x_{0,j}|>\para{1+\frac{1}{\sqrt{1-\delta_k^-}}}\|\ep\|_2$ for all $j\in S$ then the oracle solution $x'=x_S$ is a strict local minimizer of $\ksir$ with $\supp (x')=\supp (x_0)$. This also satisfies $|x'_j|>\|\epsilon\|_2$, $j\in S$, $\|Ax'-b\|_2\leq \|\epsilon\|_2$ and $$\|x'-x_0\|_2\leq \frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}.$$
\end{proposition}

\begin{proof}
We assume for simplicity that we work over $\R$, and as in Proposition \ref{p1} we let $x'$ be the oracle solution. All estimates of Proposition \ref{p1} go through with minor modifications, for example \eqref{sofg} is replaced by \begin{equation}\label{hy}|x_{j}'|\geq |x_{0,j}|-|\de_j|>|x_{0,j}|-\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}},\quad j\in S\end{equation} which shows that $\supp (x')=\supp (x_0)$ as well as $|x'_j|>\|\epsilon\|_2$ for $j\in S$.
The only real difference is the proof that $x'$ is a local minimizer of $\ksir$, so we consider $\ksir(x'+v)$ where as usual we can assume that $x'=|\tilde x'|$. Since $x'$ solves the least squares problem posed initially, the vector $A_S^*(Ax'-b)=A_S^*(A_Sx'-b)$ must be 0, and so \begin{equation*}\ksir(x'+v)=\Q_2(\iota_{P_k})(x'+v)+2\sum_{j=k+1}^n v_j\scal{a_j,Ax'-b} +\|Av\|_2^2+\ksir(x').\end{equation*} Let $k_1$ be such that $x_{k+1-k_1}=x_k$ but $x_{k-k_1}>x_k$, and note that $k_*$ will depend on $v$ but will always satisfy $k_*\leq k_1$. With this in mind $\Q_2(\iota_{P_k})(x'+v)$ becomes \[\begin{split} & \frac{1}{k_*}\left(k_*x_k+\sum_{j=k-k_*+1}^k v_j+\sum_{j=k+1}^n|v_j|\right)^2-\sum_{j=k-k_*+1}^k(x_k+v_j)^2-\sum_{j=k+1}^n v_j^2 \\ & = k_* x_k ^2 + 2 x_k \sum_{j=k-k_*+1}^k v_j + 2 x_k \sum_{j=k+1}^n |v_j| - k_* x_k ^2 -  2 x_k \sum_{j=k-k_*+1}^k v_j + P(v)  \end{split}\] where \(P(v) \) is a quadratic function in \(v\) only. Therefore after the cancellations we are left with
$2x_k\sum_{j=k+1}^n|v_j|$ plus quadratic terms in $v$.
Returning to the expression for $\ksir(x'+v)$ and collecting all quadratic contributions from $v$ in a term $q(v)$, we see that $\ksir(x'+v)-\ksi(x')$ equals
\begin{equation*}2x_k\left(\sum_{j=k+1}^n|v_j|\right)+2\left(\sum_{j=k+1}^n v_j\scal{a_j,Ax'-b}\right) +q(v).\end{equation*}
Since $|\scal{a_j,Ax'-b}|\leq\|\epsilon\|_2$ and $x_k>\|\epsilon\|_2$, it is easy to see that there exist some constant $\rho>0$ such that \begin{equation*}2x_k\left(\sum_{j=k+1}^n|v_j|\right)+2\left(\sum_{j=k+1}^n v_j\scal{a_j,Ax'-b}\right)\geq\rho\sqrt{\sum_{j=k+1}^nv_j^2}\end{equation*} for \(v\) in a neighborhood of $0$. As in the proof of Proposition \ref{p1} we conclude that we must have $\sum_{j=k+1}^nv_j^2=0$ in order for $\ksir(x'+v)\leq \ksir(x')$ to be possible. However, for $v$ with $\supp v\subset S,$ $\Q_2(\iota_{P_k})(x'+v)=0$ and so $$\ksir(x'+v)=\|A(x'+v)-b\|_2^2\geq \|Ax'-b\|_2^2=\ksir(x'),$$ and the proof is complete.




\end{proof}

To go from saying that $x'$ is a strict local minimizer to saying unique global minimizer is now a short step.

\begin{theorem}\label{cor:dogadgetf}
Let $A$ be $k$-feasible and $\delta_{2k}^->1/{2}$. If $$|x_{0,j}|>\para{\frac{1}{1-2\delta_{2k}^-}+\frac{1}{\sqrt{1-\delta_k^-}}}\|\ep\|_2,\quad j\in S$$ then the oracle solution $x'$ in the above proposition is a global minimum of $\ksi$ and $\ksir$. Moreover, if $A$ is strictly $k$-feasible then $\ksir$ has no other local minimizers.
\end{theorem}
\begin{proof}
Proposition \ref{p1f} clearly applies and  ensures that $x'$ is a local minimizer. We now check that \eqref{e4fix} applies for $z'$ given by \eqref{y}, i.e. we want to check that $|\tilde z'_{k+1}|<(1-2\delta_{2k}^-)|\tilde z'_k|$. Note that $|\tilde z'_{k+1}|\leq\|\ep\|_2$ by the same estimate as \eqref{o0}. Moreover, since $z'\in\partial \G(x')$, Lemma \ref{sun} implies that it suffices to show that $\|\ep\|_2<(1-2\delta_{2k}^-)|\tilde x'_k|$, which by \eqref{hy} follows if
$$\|\ep\|_2<(1-2\delta_{2k}^-)\para{|\tilde x_{0,k}|-\frac{\|\ep\|_2}{\sqrt{1-\delta_k^-}}}$$ which easily is seen to be equivalent with the condition in the statement. The desired conclusions now follow by Theorem \ref{thm:globalpoint2f}.
\end{proof}


